Fast Quantization of Stochastic Volatility Models

Recursive Marginal Quantization (RMQ) allows fast approximation of solutions to stochastic differential equations in one-dimension. When applied to two factor models, RMQ is inefficient due to the fact that the optimization problem is usually performed using stochastic methods, e.g., Lloyd's algorithm or Competitive Learning Vector Quantization. In this paper, a new algorithm is proposed that allows RMQ to be applied to two-factor stochastic volatility models, which retains the efficiency of gradient-descent techniques. By margining over potential realizations of the volatility process, a significant decrease in computational effort is achieved when compared to current quantization methods. Additionally, techniques for modelling the correct zero-boundary behaviour are used to allow the new algorithm to be applied to cases where the previous methods would fail. The proposed technique is illustrated for European options on the Heston and Stein-Stein models, while a more thorough application is considered in the case of the popular SABR model, where various exotic options are also priced.

==> Sections/SABR.tex <==
%!TEX root = ../Fast Quantization of SV Models.tex
In the notation of equations \eqref{Eq: X-process} and \eqref{Eq: Y-process}, the SABR model is decribed by
\begin{align}
a^x(X_t) &= 0, & &b^x(X_t) = \nu X_t, \\
a^y(Y_t) &= 0, & &b^y(X_t, Y_t) = X_t C(Y_t),
\end{align}
with $C(Y_t)$, known as the \emph{backbone} function, most commonly taken to be an offset CEV factor,
\[ C(Y_t) = (Y_t + o)^\beta \]
with $0\leq\beta\leq1$. This is the case we consider here, and without loss of generality, we set the offset, $o$, to zero.

A partial reason for the popularity of the SABR model is the existence of a closed-form formula for the implied volatility, provided in the original paper by \cite{hagan2002managing}. Further work has extended the formula and corrected various biases (see, for example, \cite{obloj2007fine} and \cite{paulot2015asymptotic}).
The latest version is given in \cite{hagan2016universal} and applies to all potential specifications of the backbone function.

\subsection{European Options}
\label{Sec: SABR European Options}
In this section, we consider European options for two examples of extreme parameter sets that could arise in the context of interest rate modelling.
Although the RMQ algorithm would not be used in cases where accurate closed-form approximations are available, these examples illustrate its flexibility and important aspects of its convergence.

\begin{figure}[t!]
     \begin{center}
         \includegraphics[width=\columnwidth]{Figures/Plot_chen_SABR}
     \end{center}
     \caption{Implied Bachelier volatility and pricing error for the standard SABR model, using a parameter set suited for an interest rate environment.}
     \label{Fig: Plot_chen_SABR}
\end{figure}

In Figure \ref{Fig: Plot_chen_SABR}, $\beta = 0.7$, $\nu=0.3$, $\rho=-0.3$, $X_0 = 20\%$, $Y_0=0.5\%$ and the maturity of the option is set at one year.
This parameter set forms Test Case III from \cite{chen2012efficient}, and was specifically chosen to be appropriate to the fixed income market and to make the effect of the zero-boundary behaviour clearly observable. The reference price is provided by the implied volatility formula from \cite{hagan2016universal} with the boundary correction specified in that work. 

For the RMQ algorithm, $24$ timesteps were taken and $30$ codewords were used at each step for both processes, i.e., $N^y = N^x = 30$ for $1\leq k \leq 24$. 
A reflecting boundary was implemented for the dependent process. The Monte Carlo simulation utilized a fully-truncated Euler discretization scheme with $240$ time-steps and $500\,000$ paths.

There are two things to note for this example. Firstly, there is significant bias in the Monte Carlo scheme. This can be seen in the three standard deviation bound plotted on the right-hand side of Figure \ref{Fig: Plot_chen_SABR}. It indicates that the Monte Carlo simulation is not converging to the same result as the \cite{hagan2016universal} implied volatility, used here to determine the reference price. In their discussion, \cite{chen2012efficient} indicate that this is a challenging parameter set for traditional Monte Carlo simulation. Secondly, the RMQ algorithm is highly accurate, despite the low number of codewords and the coarseness of the resulting grid.

In this case, it is also significantly faster to compute than the Monte Carlo simulation. On a $2.00$ GHz Intel i-$3$ with $4$ GB of RAM, the MATLAB implementation of the RMQ algorithm took approximately $10.8$ seconds, whereas the Monte Carlo simulation took $24.6$ seconds, owing to the much larger amount of timesteps. For this example, the same paths were used to price all strikes, as independent errors disrupt the smoothness of the smile. The results do not change significantly when unique paths are generated for each strike.
 

\begin{figure}[t!]
     \begin{center}
         \includegraphics[width=\columnwidth]{Figures/Plot_normal_SABR}
     \end{center}
     \caption{Implied normal volatility and pricing error for the Bachelier SABR model.}
     \label{Fig: Plot_normal_SABR}
\end{figure}

In Figure \ref{Fig: Plot_normal_SABR}, the implied normal volatility and pricing error are displayed when using the RMQ algorithm, an Euler Monte Carlo simulation, as well as a semi-closed form solution from \cite{korn2013exact} for the \emph{Bachelier} SABR model, i.e., the case when $\beta = 0$. The other parameters are $\nu=0.3691$, $\rho=-0.0286$, $X_0 = 0.68\%$, $Y_0=4.35\%$, with the maturity of the option set at one year. This parameter set forms Test Case I from \cite{korn2013exact} and it describes a challenging simulation environment with a low initial forward rate which is very volatile.

For the RMQ algorithm, $12$ time-steps were taken along with $10$ codewords for the independent process and $90$ codewords for the dependent process. Thus, $N^x = 10$ and $N^y = 90$ for $1\leq k \leq 12$. For the Euler Monte Carlo simulation, $500\,000$ paths were used, along with $120$ time-steps.  Note that the semi-closed form solution from \cite{korn2013exact} requires the numerical solution of an integral and is computationally more expensive than the implied volatility calculation. Again, a single set of Monte Carlo paths was used to price all strikes. The RMQ algorithm took $4.3$ seconds, whereas the Monte Carlo simulation took $4.5$ seconds.

This example is notable for the high accuracy of the RMQ algorithm, despite the extreme parameter set, with all the corresponding prices falling well within the three standard deviation bound of the Monte Carlo simulation. This is owing to two factors: the conditionally normal nature of the dependent process and how the total number of codewords is distributed.

As we are using an Euler approximation to recursively quantize the process, it should be clear that the RMQ algorithm will perform well when approximating a process that itself is also conditionally Gaussian. Secondly, in the SABR case, the volatility is modelled using geometric Brownian motion. For this example, very few codewords are needed at each time-step to form a reasonably accurate quantized representation of the distribution of the volatility. Thus, the majority of the computation time can instead be spent on quantizing the conditionally Gaussian dependent process. If we instead use $30$ codewords for each process, even though the total number of codewords would be unchanged, the results are not as accurate.

\subsection{Exotic Options}
\label{Sec: SABR Exotic Options}
\begin{figure}[t!]
     \begin{center}
         \includegraphics[width=\columnwidth]{Figures/Plot_joint_prob_SABR}
     \end{center}
     \caption{Time-evolution of the approximate joint probability for the SABR model of Section \ref{Sec: SABR Exotic Options}.}
     \label{Fig: Plot_joint_prob_SABR}
\end{figure}
An advantage of the RMQ algorithm, similar to binomial and trinomial tree methods, is the ability to price many options off the grid that results from a single run. This is demonstrated in this section by using a single pass of the RMQ algorithm to price European, Bermudan and barrier options, as well as volatility corridor swaps.

The model parameters for all the examples in this section are $\beta = 0.9$, $\nu=0.4$, $\rho=-0.3$, $X_0 = 0.4$ and $Y_0=S_0\exp(rT)$, where $Y_0$ models the time-$T$ forward price of an equity asset with $S_0 = 100$ and $T$ is set at $1$ to coincide with the maturity of the options considered. For the RMQ algorithm, $24$ timesteps are used with $N^x = 30$ codewords for the volatility process and $N^y = 60$ codewords for the forward price process with $1\leq k \leq 24$.
The Monte Carlo simulations are executed using a fully-truncated Euler scheme with $120$ time-steps and $500\,000$ paths

The execution of the RMQ algorithm for these parameters takes approximately $16$ seconds on the same architecture as in Section \ref{Sec: SABR European Options}.
Figure \ref{Fig: Plot_joint_prob_SABR} illustrates the time-evolution of the approximate joint probability of the forward price of the asset and the volatility over the course of the year for the grid generated by these model parameters. By keeping the axes fixed, it highlights how the codewords spread over time owing to the increased marginal variance of each process.

\begin{figure}[t!]
     \begin{center}
         \includegraphics[width=\columnwidth]{Figures/Plot_tian_SABR1}
     \end{center}
     \caption{European and Bermudan put option prices for the SABR model in an equity framework.}
     \label{Fig: Plot_tian_SABR1}
\end{figure}

The left-hand side of Figure \ref{Fig: Plot_tian_SABR1} illustrates the error when pricing European put options on the generated grid when compared to the prices generated by the implied volatility formula of \cite{hagan2016universal}. The right-hand side shows the prices for a Bermudan put with monthly exercise opportunities priced from the generated grid as well as using a least-squares Monte Carlo simulation. For each strike, generating an option price using Monte Carlo simulation takes approximately $12$ seconds for the European options and $14$ seconds for the Bermudan options, owing to the backward pass required by the least-squares algorithm. The high-level algorithm for pricing Bermudan options using a quantization grid is outlined in \cite{mcwalter2017recursive}.

\begin{figure}[t!]
     \begin{center}
         \includegraphics[width=\columnwidth]{Figures/Plot_tian_SABR2}
     \end{center}
     \caption{Price comparison for discrete up-and-out put options and volatility corridor swaps in the SABR model.}
     \label{Fig: Plot_tian_SABR2}
\end{figure}

The left-hand side of Figure \ref{Fig: Plot_tian_SABR2} shows the RMQ and Monte Carlo prices for a discrete up-and-out put option, with monthly monitoring, where the barrier level is expressed as a multiple of the at-the-money strike. The right-hand side shows the prices for a series of volatility corridor swaps. The payoff of a volatility corridor swap is given by
\begin{align}
 \frac{1}{T}\int_0^T X_z \ind{L < S_z < H}\, dz \label{Eq: Volatility Corridor Swap Payoff}
\end{align}
where $S_t = Y_t\exp(-r(T - t))$ is the asset price in our deterministic interest-rate framework and $L$ and $U$ specify the \emph{corridor} of the asset price in which the volatility is accumulated. The algorithm for pricing volatility corridor swaps on a quantization grid in the stochastic volatility setting is presented in \cite{callegaro2015pricing} and used here without modification. 

The corridor spreads on the $x$-axis represent a percentage bound around the initial asset price value, i.e., the lower bound of the corridor is given by $L = S_0(1 - s)$ and the upper bound by $U = S_0(1 + s)$ where $s$ is the corridor spread. The vertical gap between the prices generated by the Monte Carlo simulation and the RMQ algorithm is partially owing to the increased accuracy obtained in the Monte Carlo simulation when using simple quadrature to approximate Equation \eqref{Eq: Volatility Corridor Swap Payoff}, because of the increased number of time-steps. For a single barrier value or a single corridor spread, the Monte Carlo simulation takes approximately $13$ seconds to price the considered option. 
